Spatiotemporal Dependable Task Execution Services in MEC-enabled Wireless Systems

Multi-access Edge Computing (MEC) enables computation and energy-constrained devices to offload and execute their tasks on powerful servers. Due to the scarce nature of the spectral and computation resources, it is important to jointly consider i) contention-based communications for task offloading and ii) parallel computing and occupation of failure-prone MEC processing resources (virtual machines). The feasibility of task offloading and successful task execution with virtually no failures during the operation time needs to be investigated collectively from a combined point of view. To this end, this letter proposes a novel spatiotemporal framework that utilizes stochastic geometry and continuous time Markov chains to jointly characterize the communication and computation performance of dependable MEC-enabled wireless systems. Based on the designed framework, we evaluate the influence of various system parameters on different dependability metrics such as (i) computation resources availability, (ii) task execution retainability, and (iii) task execution capacity. Our findings showcase that there exists an optimal number of virtual machines for parallel computing at the MEC server to maximize the task execution capacity.

==> system_model/system_model_old.tex <==
% !TEX root =../Integration.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{System Model}\label{sec:system_model}

In this work, we consider a cellular uplink network, where the devices are spatially dropped in $\mathbb{R}^2$ according to a homogeneous \acp{PPP}, denoted by $\mathrm{\Phi}$ with intensity $\lambda_d$ devices/unit area. A single cell scenario where the \ac{BS}, accompanied with a physically co-located \ac{MEC} server, is deployed at the center with circular radio coverage area equals $A=\pi R^2$. \footnote{Thus, the total number of devices $N_d$ within the deployment area $A$ follows a Poisson distribution with intensity $N_d = \pi R^2 \lambda_d$.} An unbounded path-loss propagation model is adopted such that the signal power attenuates at the rate $r^{-\eta}$, where $r$ is the distance and $\eta > 2$ is the path-loss exponent. Small-scale fading is assumed to be multi-path Rayleigh fading, where the signal of interest and interference channel power gains $h$ and $g$, respectively, are exponentially distributed with unit power gain. All channel gains are assumed to be spatially and temporally independent and identical distributed (i.i.d.). Full path-loss channel-inversion power control is adopted, which implies that all devices adjust their transmit powers such that the received uplink average powers at the \ac{BS} is equal to a predetermined value $\rho$ \cite{ElSawy2014}. 

\begin{figure}
	\begin{center}
		\includegraphics[width=\columnwidth]{system_model/figures/MEC_oper_model/MEC_oper_model.eps}
		\caption{Spatiotemporal network realization for devices with no generated, locally or offloaded tasks.} 
		\label{fig:system_model}
	\end{center}
\end{figure}

Regarding the temporal parameters, we consider a continuous time system with task transmission duration equals $T_s$ seconds. Task arrivals at the devices are modeled via a Poisson process with rate $\lambda_a$ task/unit time\cite{Ko2018}. Upon their arrivals, devices attempt to transmit the corresponding task to the \ac{BS} via uplink to be centrally processed at the \ac{MEC} server.  Each device selects  randomly one of $C$ available channels at the \ac{BS} to transmit its task via uplink communication. Such a task is successfully received (i.e., decoded) at the \ac{BS} if the received \ac{SINR} is larger than a predefined threshold $\theta$. The \ac{TSP} of a generic device, which is denoted by $p_o$, quantifies the probability of successful decoding as $ p_o= \mathbb{P}\{\text{SINR}_o>\theta\}$. \footnote{Acknowledgment for successful transmission is ignored as it incurs negligible time compared $T_s$.} In case of failed transmission, the device proceeds to compute its task locally. Accordingly, we adopt a coverage-based offloading criteria in our framework, whereas the \ac{TSP} $p$ governs the offloading decision.  

Moving to the computation parameters, the \ac{MEC} server is equipped with a \ac{PM} that employs parallel computing of tasks by creating a number of \acp{VM}. Furthermore, we consider a static \acp{VM}-generation, where a fixed number, denoted by $M$, \acp{VM} are employed. Based on the shared computation resources within the \ac{PM} (e.g., buses for I/O, CPU, memory), I/O interference is observed within the \ac{PM}, where simultaneous \acp{VM} can interfere with each other with some cost on their computational power \cite{Bruneo2014}. In our model, each task and its subsequent segments can occupy at most one \ac{VM}. In case of a single \ac{VM}, we model the computational time of a \ac{VM} via a Poisson process with rate $\mu_o$ task/unit time. To account for the I/O interference, the computational rate of of any of the $M$ \acp{VM} depends on the total number of \acp{VM} as follows
\begin{equation}
\mu_{\text{MEC}} = \frac{\mu_o}{(1+d)^{M-1}},
\end{equation}
where $d$ is the degradation factor due to I/O interference between the M \acp{VM} \cite{Ko2018, Bruneo2014}. Devices are assumed to be equipped with a local \ac{PM} that can at most employ one virtual machine, where the computational time of such \ac{VM} is modeled via a Poisson process with rate $\mu_{\text{loc}}$. To investigate the relative ratio between the centralized and the local computational capabilities, we let $\mu_r = \frac{\mu_{\text{MEC}} }{\mu_{\text{loc}}}$ denote the relative service rate such that $\mu_r >> 1$.

To account for the hardware and software failures in the \ac{PM} and its different \acp{VM} \cite{Fu2009,Birke2014}, our proposed model takes into account events of \acp{VM} failures and the time required to ensure successful repair. We model the failure (repair) rate of a given \ac{VM} via a Poisson process with rate $\delta$ ($\gamma$) VM/unit time. \acp{VM} are prone to failure whether they are idle (not currently computing a task) or occupied. The former is considered to model hardware and I/O failures, while the latter takes into account hardware and software events that might to cause the \ac{VM} to halt its operation. In case of failure of an idle \ac{VM}, this \ac{VM} is labeled as \ac{OoO} and cannot admit future tasks. In case of an occupied \ac{VM} failure, the \ac{PM} will handover the running task to an idle \ac{VM}, if one exists. If not, the task will be discarded and the device will be notified via downlink. A pictorial visualization of our system is as shown in Fig. \ref{fig:system_model}, where a number of devices in the network are labeled as active or idle depending on their temporal activities. The active devices offload their tasks to the MEC server, where they are computed. For the red-labeled task, failure occurs while being in service, thus, this task is offloaded to a free \ac{VM} to resume its computation. Based on the repair rate, the failed \ac{VM} goes back into operation to accommodate future incoming arrivals. 

==> system_model/system_model_old_old.tex <==
% !TEX root =../Integration.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{System Model}\label{sec:system_model}

In this work, we consider the execution of computational tasks generated by a device, either locally (i.e., utilizing the devices computational resources), or by offloading them to  remote cloud server, through a wireless transmission resource. First, the physical and medium access control (MAC) parameters are presented in subsections \ref{sec:PHY} and \ref{sec:MAC}, respectively. The tasks generation, execution and components are then discussed in subsection \ref{sec:TG}.  

\subsection{Spatial and Physical Layer Parameters}\label{sec:PHY}
In this work, we consider a cellular uplink network, where the \acp{BS} and the devices are spatially deployed in $\mathbb{R}^2$ according to two independent homogeneous \acp{PPP}, denoted by $\mathrm{\Psi}$ and $\mathrm{\Phi}$ with intensities $\lambda$ and $\mu$, respectively. The devices in our framework are left generic to mimic a wide range of use cases as explored in Fig. \ref{fig:used_cases}. Every device is equipped with a local processing unit with processing power $C_l$, measured in cycles/sec, that can execute the generated tasks locally. In addition. at each BS in the network, a \ac{MEC} server is co-located, with total processing power $C_M$, measured cycles/second. Thus, devices can offload their tasks to their serving BS/MEC, leveraging its larger processing power and closer proximity. Single antennas are employed at all devices and \acp{BS}. Uplink configured-grant is adopted aligning with 3GPP release 16 which allows the devices to autonomously transmit data without having to send a scheduling request and wait for the uplink grant. Thus, devices attempt their transmissions on a randomly selected channel without a scheduling grant from their serving \ac{BS}. In particular, a set of $N_c$ channels are utilized by every \ac{BS} within the network, where every device is granted a channel for its transmission. Single connectivity is considered where each device is served by its nearest \ac{BS}. 

An unbounded path-loss propagation model is adopted such that the signal power attenuates at the rate $r^{-\eta}$, where $r$ is the distance and $\eta > 2$ is the path-loss exponent. Small-scale fading is assumed to be multi-path Rayleigh fading, where the signal of interest and interference channel power gains $h$ and $g$, respectively, are exponentially distributed with unit power gain. All channel gains are assumed to be spatially and temporally independent and identical distributed (i.i.d.). Full path-loss channel-inversion power control is adopted, which implies that all devices adjust their transmit powers such that the received uplink average powers at their serving \ac{BS} is equal to a predetermined value $\rho$ \cite{ElSawy2014}. Moreover, a dense deployment of \acp{BS} is assumed, ensuring that every device is able to invert its path-loss almost surely.

\begin{figure*}
	\centering
	\ifCLASSOPTIONdraftcls
	\input{system_model/figures/1col/deployment.tex}
	\vspace{-0.4in}
	\else
	\input{system_model/figures/2col/deployment.tex}
	\fi 		
	\caption{Spatiotemporal network realization with $\lambda = 0.002$ BS/km$^2$, $\mu=0.01$ device/km$^2$ and $\gamma=0.5$. Solid blue lines and dashed magenta lines show coverage regions and associations, respectively.} 
	\label{fig:interf_per}
\end{figure*}

 A packet generated at a given device is successfully received at its serving \ac{BS} if the received \ac{SINR} is larger than a predefined threshold $\theta$. In addition,let $p_i$ denotes  the coverage probability of the $i$-th device, which is evaluated as $ = \mathbb{P}\{\text{SINR}_i>\theta\}$. In the case of successful reception, the serving \ac{BS} transmits an ACK so the device can remove this intended packet from its respective queue. In the case of failed decoding, the serving \ac{BS} sends out an NACK and the packet remains at the head of the device's queue, awaiting a new transmission attempt in the next time slot. In this work, we assume error-free and negligible delay for ACK and NACK.
 
\subsection{MAC Layer Parameters}\label{sec:MAC}

The proposed framework considers a synchronized and time slotted system with slot duration $T_s$ [s]. A fixed transmission rate of $R_f=\log_2(1+\theta)$ measured in bits/second is considered, such that a packet of size $T_sR_f$ is successfully transmitted at the serving BS (intended device) for uplink (downlink) transmission. A potential device opts to offload its generated task to its serving BS, that has a \ac{MEC} server physically co-located with it, based on the parameter $\alpha \ in (0,1]$, which is a bias factor to control traffic offloading from the local to the centralized-cellular entities (\textcolor{red}{Here the additional location-aware offloading criteria should be introduced}). On one extreme, setting $\alpha=0$ disables the local execution of tasks. On the other extreme, setting
$\alpha=1$ forces all devices with tasks in their queues to offload them to their serving BSs. 

\subsection{Task generation and execution}\label{Sec:TG}

In the considered framework tasks are generated at a given device based on an a Bernoulli task generation model, with per-slot task arrival probability of $\gamma \in (0,1]$. A generic task $i$ is characterized by the tuple $\mathbf{\Omega}_i = (\tau_i, f_i, \ell_{in,i}, \ell_{out,i})$, where $\tau_i$ is the task's anticipated deadline measured in time slot, $f_i$ is the number of processing operations per input bit required measured in cycles/bit and $\ell_{in,i}$ ($\ell_{out,i}$) is the number of input  (output) bits.  
When task offloading is carried out, $\ell_{in,i}$ and $\ell_{out,i}$ represent task input and output bits that are transmitted through a wireless channel via uplink and downlink, respectively. However, for local execution, $\ell_{out,i} = 0$, since no communication is carried out between the device and its serving BS/MEC server. 

As highlighted in the previous section, in order to account for the latency dependent nature of the generated tasks, each task is tagged with its completion deadline $\tau$, such that $\tau \in \{\tau_{\text{min}}, \tau_{\text{min}+1},\cdots, \tau_{\text{max}+1}-1, \tau_{\text{max}}\}$, where $\tau_{\text{min}}$ and $\tau_{\text{max}}$ represent the minimum and maximum allowable task deadlines. To account for the tasks heterogeneity, we consider that the deadlines vary across different tasks such that $\tau$ is drawn from a discrete distribution $f_{\tau}(t)$ in the range of $\tau_{\text{min}} \leq \tau_{\text{max}}$. Accordingly, a task is labeled as \textit{timed out} if not completed within $\tau$ time slots from its time of generation. On the contrary, successful task completion implies that the device has successfully executed the task, either locally, or via offloading before its deadline. 
\subsubsection{Local Execution}
Assuming that the $i$-th device opts to execute a task locally, the total local execution time is evaluated as
\begin{equation}
T_{\text{local},i} = \frac{\ell_{in,i}f_i}{C_l}.
\end{equation} 
\subsubsection{Offloaded Execution}
For the case that the $i$-th device opts to offload its task to the $j$-th BS, the total offloading execution time is evaluated as
\begin{equation}\label{eq:Texc_offload}
T_{\text{off},i} = \underbrace{\frac{\ell_{in,i}}{r_{\text{UL},i}}}_{\text{uplink latency} }+\underbrace{ \frac{\ell_{in,i}f_i}{C_M}}_{\text{execution latency}}+\underbrace{\frac{\ell_{out,i}}{r_{\text{DL},i}}}_{\text{downlink latency}}, 
\end{equation} 
where $r_{\text{UL},i}$ and $r_{\text{DL},i}$ represent the transmission rate of the $i$-th task for uplink and downlink transmission, respectively. Similar to the local execution, let $s_{o,i}$ be the probability of successful execution of the $i$-th task given that it was offloaded to its serving BS/MEC server, which equals
\begin{equation}\label{eq:Texc_off}
s_{o,i} = \mathbb{P}\{T_{\text{off},i} < \tau_i\}. 
\end{equation}
